A Global Model of The Light Curves and Expansion Velocities of Type II-Plateau Supernovae

We present a new self-consistent and versatile method that derives photospheric radius and temperature variations of Type II-Plateau supernovae based on their expansion velocities and photometric measurements. We apply the method to a sample of 26 well-observed, nearby supernovae with published light curves and velocities. We simultaneously fit ~230 velocity and ~6800 magnitude measurements distributed over 21 photometric passbands spanning wavelengths from 0.19 to 2.2 microns. The light curve differences among the Type II-Plateau supernovae are well-modeled by assuming different rates of photospheric radius expansion, which we explain as different density profiles of the ejecta and we argue that steeper density profiles result in flatter plateaus, if everything else remains unchanged. The steep luminosity decline of Type II-Linear supernovae is due to fast evolution of the photospheric temperature, which we verify with a successful fit of SN1980K. Eliminating the need for theoretical supernova atmosphere models, we obtain self-consistent relative distances, reddenings, and nickel masses fully accounting for all internal model uncertainties and covariances. We use our global fit to estimate the time evolution of any missing band tailored specifically for each supernova and we construct spectral energy distributions and bolometric light curves. We produce bolometric corrections for all filter combinations in our sample. We compare our model to the theoretical dilution factors and find good agreement for the B and V filters. Our results differ from the theory when the I, J, H, or K bands are included. We investigate the reddening law towards our supernovae and find reasonable agreement with standard R_V ~ 3.1 reddening law in UBVRI bands. Results for other bands are inconclusive. We make our fitting code publicly available.

==> bc.tex <==
$U - B$ &  $(-1.27, 1.46)$ &  $ -0.3222 $ &  $ -0.3297 $ &  $  0.0383 $ &  $  0.2977 $ &  $ -0.4111 $ & $   0.162 $ \\
$U - V$ &  $(-1.54, 2.74)$ &  $  0.0691 $ &  $  0.2461 $ &  $ -0.2797 $ &  $  0.1561 $ &  $ -0.0314 $ & $   0.021 $ \\
$U - R$ &  $(-1.53, 3.53)$ &  $  0.1871 $ &  $  0.4333 $ &  $ -0.3031 $ &  $  0.1153 $ &  $ -0.0158 $ & $   0.024 $ \\
$U - I$ &  $(-1.63, 3.87)$ &  $  0.1943 $ &  $  0.4891 $ &  $ -0.2744 $ &  $  0.0863 $ &  $ -0.0094 $ & $   0.031 $ \\
$U - J$ &  $(-1.73, 4.17)$ &  $  0.2021 $ &  $  0.5331 $ &  $ -0.2434 $ &  $  0.0691 $ &  $ -0.0068 $ & $   0.033 $ \\
$U - H$ &  $(-1.67, 4.09)$ &  $  0.2460 $ &  $  0.5701 $ &  $ -0.2461 $ &  $  0.0785 $ &  $ -0.0097 $ & $   0.020 $ \\
$U - K$ &  $(-1.57, 4.38)$ &  $  0.2863 $ &  $  0.6475 $ &  $ -0.2749 $ &  $  0.0681 $ &  $ -0.0061 $ & $   0.035 $ \\
$U - g$ &  $(-1.42, 2.34)$ &  $ -0.0373 $ &  $  0.0369 $ &  $ -0.3068 $ &  $  0.2238 $ &  $ -0.0575 $ & $   0.024 $ \\
$U - r$ &  $(-1.64, 3.36)$ &  $  0.1052 $ &  $  0.3484 $ &  $ -0.2701 $ &  $  0.1104 $ &  $ -0.0159 $ & $   0.026 $ \\
$U - i$ &  $(-1.93, 3.41)$ &  $ -0.0220 $ &  $  0.3069 $ &  $ -0.1836 $ &  $  0.0833 $ &  $ -0.0129 $ & $   0.024 $ \\
$U - z$ &  $(-2.20, 3.64)$ &  $ -0.0837 $ &  $  0.3260 $ &  $ -0.1608 $ &  $  0.0572 $ &  $ -0.0063 $ & $   0.036 $ \\
$uvw2 - U$ &  $(-1.37, 2.19)$ &  $  0.3854 $ &  $  0.1288 $ &  $ -0.1786 $ &  $  0.0098 $ &  $ -0.0046 $ & $   0.002 $ \\
$uvm2 - U$ &  $(-2.12, 2.56)$ &  $  0.4056 $ &  $  0.0378 $ &  $ -0.0985 $ &  $  0.0023 $ &  $ -0.0014 $ & $   0.002 $ \\
$uvw1 - U$ &  $(-1.11, 1.32)$ &  $  0.4058 $ &  $  0.0703 $ &  $ -0.3613 $ &  $  0.0144 $ &  $ -0.0198 $ & $   0.002 $ \\
$u - U$ &  $(-0.64, 0.35)$ &  $  0.1829 $ &  $ -1.6143 $ &  $ -3.4435 $ &  $ -2.8074 $ &  $ -4.3188 $ & $   0.014 $ \\
$U - b$ &  $(-1.23, 0.90)$ &  $ -0.2415 $ &  $ -0.3491 $ &  $ -0.2551 $ &  $  0.3189 $ &  $ -0.2645 $ & $   0.005 $ \\
$U - v$ &  $(-1.58, 1.75)$ &  $  0.0601 $ &  $  0.2695 $ &  $ -0.2332 $ &  $  0.1355 $ &  $ -0.0414 $ & $   0.005 $ \\
$B - V$ &  $(-0.26, 1.27)$ &  $ -0.3716 $ &  $  2.9669 $ &  $ -6.2797 $ &  $  5.8950 $ &  $ -2.0233 $ & $   0.023 $ \\
$B - R$ &  $(-0.25, 2.06)$ &  $ -0.5660 $ &  $  3.1858 $ &  $ -3.8405 $ &  $  2.1115 $ &  $ -0.4220 $ & $   0.028 $ \\
$B - I$ &  $(-0.35, 2.40)$ &  $ -0.4779 $ &  $  2.5717 $ &  $ -2.5096 $ &  $  1.1576 $ &  $ -0.1914 $ & $   0.030 $ \\
$B - J$ &  $(-0.46, 2.71)$ &  $ -0.4194 $ &  $  2.1902 $ &  $ -1.7737 $ &  $  0.7316 $ &  $ -0.1086 $ & $   0.030 $ \\
$B - H$ &  $(-0.40, 2.63)$ &  $ -0.5115 $ &  $  2.4165 $ &  $ -1.9163 $ &  $  0.8285 $ &  $ -0.1372 $ & $   0.023 $ \\
$B - K$ &  $(-0.30, 2.91)$ &  $ -0.6888 $ &  $  2.7924 $ &  $ -1.9578 $ &  $  0.6777 $ &  $ -0.0860 $ & $   0.032 $ \\
$B - g$ &  $(-0.15, 0.88)$ &  $ -0.3901 $ &  $  4.5522 $ &  $ -18.0611 $ &  $ 25.8333 $ &  $ -13.0179 $ & $   0.029 $ \\
$B - r$ &  $(-0.36, 1.90)$ &  $ -0.3536 $ &  $  2.3983 $ &  $ -3.3400 $ &  $  2.0798 $ &  $ -0.4617 $ & $   0.029 $ \\
$B - i$ &  $(-0.66, 1.95)$ &  $ -0.1890 $ &  $  1.2111 $ &  $ -1.5985 $ &  $  1.1468 $ &  $ -0.2868 $ & $   0.027 $ \\
$B - z$ &  $(-0.92, 2.17)$ &  $ -0.1817 $ &  $  0.9171 $ &  $ -0.9199 $ &  $  0.5572 $ &  $ -0.1131 $ & $   0.031 $ \\
$uvw2 - B$ &  $(-2.65, 3.09)$ &  $ -0.3038 $ &  $  0.1656 $ &  $ -0.0749 $ &  $  0.0062 $ &  $ -0.0014 $ & $   0.005 $ \\
$uvm2 - B$ &  $(-3.40, 3.45)$ &  $ -0.2936 $ &  $  0.1259 $ &  $ -0.0484 $ &  $  0.0027 $ &  $ -0.0005 $ & $   0.003 $ \\
$uvw1 - B$ &  $(-2.39, 2.22)$ &  $ -0.2425 $ &  $  0.1281 $ &  $ -0.1106 $ &  $  0.0087 $ &  $ -0.0047 $ & $   0.007 $ \\
$u - B$ &  $(-1.92, 1.23)$ &  $ -0.2388 $ &  $ -0.1580 $ &  $ -0.1864 $ &  $  0.0499 $ &  $ -0.0351 $ & $   0.001 $ \\
$B - v$ &  $(-0.30, 0.87)$ &  $ -0.3497 $ &  $  2.5231 $ &  $ -5.0024 $ &  $  5.2187 $ &  $ -2.3335 $ & $   0.003 $ \\
$V - R$ &  $( 0.01, 0.79)$ &  $ -1.7603 $ &  $ 20.1355 $ &  $ -64.9295 $ &  $ 90.8237 $ &  $ -45.9550 $ & $   0.042 $ \\
$V - I$ &  $(-0.09, 1.13)$ &  $ -0.7976 $ &  $  8.3139 $ &  $ -18.3836 $ &  $ 18.6650 $ &  $ -6.8676 $ & $   0.038 $ \\
$V - J$ &  $(-0.19, 1.43)$ &  $ -0.5059 $ &  $  5.0720 $ &  $ -8.1752 $ &  $  6.6895 $ &  $ -2.0151 $ & $   0.035 $ \\
$V - H$ &  $(-0.13, 1.35)$ &  $ -0.8370 $ &  $  5.9853 $ &  $ -9.0908 $ &  $  7.3947 $ &  $ -2.3422 $ & $   0.027 $ \\
$V - K$ &  $(-0.03, 1.64)$ &  $ -1.4387 $ &  $  7.7264 $ &  $ -9.9138 $ &  $  6.2030 $ &  $ -1.4582 $ & $   0.031 $ \\
$g - V$ &  $(-0.12, 0.39)$ &  $ -0.3530 $ &  $  6.4875 $ &  $ -36.0435 $ &  $ 101.3281 $ &  $ -110.0957 $ & $   0.015 $ \\
$V - r$ &  $(-0.10, 0.62)$ &  $ -0.2186 $ &  $  9.0218 $ &  $ -46.6996 $ &  $ 98.5857 $ &  $ -71.5178 $ & $   0.050 $ \\
$V - i$ &  $(-0.40, 0.67)$ &  $  0.2107 $ &  $  1.0045 $ &  $ -4.0562 $ &  $ 13.4633 $ &  $ -13.5288 $ & $   0.042 $ \\
$V - z$ &  $(-0.66, 0.90)$ &  $  0.1985 $ &  $  0.8277 $ &  $ -1.3300 $ &  $  3.2389 $ &  $ -2.4351 $ & $   0.036 $ \\
$uvw2 - V$ &  $(-2.91, 4.00)$ &  $ -0.2726 $ &  $  0.2635 $ &  $ -0.0573 $ &  $  0.0064 $ &  $ -0.0003 $ & $   0.002 $ \\
$uvm2 - V$ &  $(-3.66, 4.36)$ &  $ -0.2556 $ &  $  0.2102 $ &  $ -0.0372 $ &  $  0.0033 $ &  $ -0.0001 $ & $   0.001 $ \\
$uvw1 - V$ &  $(-2.65, 3.11)$ &  $ -0.1645 $ &  $  0.2695 $ &  $ -0.0781 $ &  $  0.0123 $ &  $ -0.0011 $ & $   0.002 $ \\
$u - V$ &  $(-2.18, 2.12)$ &  $  0.0363 $ &  $  0.2093 $ &  $ -0.1195 $ &  $  0.0465 $ &  $ -0.0104 $ & $   0.002 $ \\
$b - V$ &  $(-0.31, 0.87)$ &  $ -0.2555 $ &  $  2.2410 $ &  $ -5.2329 $ &  $  6.3401 $ &  $ -3.0444 $ & $   0.006 $ \\
$R - I$ &  $(-0.10, 0.34)$ &  $  0.1111 $ &  $  9.1733 $ &  $ -67.7276 $ &  $ 265.0943 $ &  $ -370.4618 $ & $   0.029 $ \\
$R - J$ &  $(-0.20, 0.64)$ &  $  0.0958 $ &  $  4.9237 $ &  $ -16.4730 $ &  $ 33.9420 $ &  $ -25.0762 $ & $   0.025 $ \\
$R - H$ &  $(-0.14, 0.57)$ &  $ -0.3442 $ &  $  6.9596 $ &  $ -20.2301 $ &  $ 37.0276 $ &  $ -26.3903 $ & $   0.013 $ \\
$R - K$ &  $(-0.04, 0.85)$ &  $ -1.2109 $ &  $ 12.0305 $ &  $ -29.3353 $ &  $ 36.9386 $ &  $ -17.4524 $ & $   0.018 $ \\
$g - R$ &  $(-0.11, 1.18)$ &  $ -0.8083 $ &  $  6.5684 $ &  $ -13.3371 $ &  $ 12.4464 $ &  $ -4.2612 $ & $   0.024 $ \\
$R - z$ &  $(-0.67, 0.11)$ &  $  0.6311 $ &  $  1.0734 $ &  $ -5.8982 $ &  $ -26.1259 $ &  $ -37.3726 $ & $   0.028 $ \\
$uvw2 - R$ &  $(-2.90, 4.35)$ &  $ -0.1944 $ &  $  0.3018 $ &  $ -0.0554 $ &  $  0.0061 $ &  $ -0.0002 $ & $   0.001 $ \\
$uvm2 - R$ &  $(-3.65, 4.72)$ &  $ -0.1696 $ &  $  0.2413 $ &  $ -0.0359 $ &  $  0.0032 $ &  $ -0.0000 $ & $   0.001 $ \\
$uvw1 - R$ &  $(-2.64, 3.46)$ &  $ -0.0762 $ &  $  0.3210 $ &  $ -0.0757 $ &  $  0.0117 $ &  $ -0.0006 $ & $   0.001 $ \\
$u - R$ &  $(-2.17, 2.47)$ &  $  0.1627 $ &  $  0.3065 $ &  $ -0.1238 $ &  $  0.0429 $ &  $ -0.0077 $ & $   0.002 $ \\
$b - R$ &  $(-0.30, 1.22)$ &  $ -0.4005 $ &  $  2.7006 $ &  $ -3.9557 $ &  $  3.1611 $ &  $ -1.0059 $ & $   0.005 $ \\
$I - J$ &  $(-0.10, 0.30)$ &  $  0.0745 $ &  $  9.6386 $ &  $ -64.0186 $ &  $ 253.3250 $ &  $ -351.3156 $ & $   0.027 $ \\
$I - K$ &  $( 0.06, 0.51)$ &  $ -3.7485 $ &  $ 41.9930 $ &  $ -161.1470 $ &  $ 298.0979 $ &  $ -204.5939 $ & $   0.022 $ \\
$g - I$ &  $(-0.21, 1.52)$ &  $ -0.5612 $ &  $  4.2988 $ &  $ -6.6033 $ &  $  4.8715 $ &  $ -1.2977 $ & $   0.026 $ \\
$r - I$ &  $( 0.01, 0.50)$ &  $ -2.0046 $ &  $ 28.8762 $ &  $ -128.6833 $ &  $ 266.4928 $ &  $ -202.8548 $ & $   0.023 $ \\
$uvw2 - I$ &  $(-3.00, 4.49)$ &  $ -0.2151 $ &  $  0.3156 $ &  $ -0.0524 $ &  $  0.0057 $ &  $ -0.0001 $ & $   0.002 $ \\
$uvm2 - I$ &  $(-3.75, 4.85)$ &  $ -0.1910 $ &  $  0.2545 $ &  $ -0.0342 $ &  $  0.0032 $ &  $ -0.0000 $ & $   0.002 $ \\
$uvw1 - I$ &  $(-2.74, 3.60)$ &  $ -0.0893 $ &  $  0.3387 $ &  $ -0.0705 $ &  $  0.0109 $ &  $ -0.0004 $ & $   0.002 $ \\
$u - I$ &  $(-2.27, 2.61)$ &  $  0.1689 $ &  $  0.3419 $ &  $ -0.1131 $ &  $  0.0374 $ &  $ -0.0063 $ & $   0.002 $ \\
$b - I$ &  $(-0.40, 1.36)$ &  $ -0.3391 $ &  $  2.1944 $ &  $ -2.6142 $ &  $  1.8670 $ &  $ -0.5405 $ & $   0.005 $ \\
$g - J$ &  $(-0.31, 1.83)$ &  $ -0.4372 $ &  $  3.2293 $ &  $ -3.8834 $ &  $  2.4416 $ &  $ -0.5557 $ & $   0.025 $ \\
$r - J$ &  $(-0.09, 0.81)$ &  $ -0.7617 $ &  $  9.2798 $ &  $ -25.1105 $ &  $ 34.6838 $ &  $ -17.4462 $ & $   0.023 $ \\
$i - J$ &  $( 0.20, 0.76)$ &  $ -12.3905 $ &  $ 89.0542 $ &  $ -239.0328 $ &  $ 296.0025 $ &  $ -137.9219 $ & $   0.035 $ \\
$uvw2 - J$ &  $(-3.10, 4.66)$ &  $ -0.2330 $ &  $  0.3308 $ &  $ -0.0496 $ &  $  0.0054 $ &  $  0.0000 $ & $   0.004 $ \\
$uvm2 - J$ &  $(-3.85, 5.04)$ &  $ -0.2093 $ &  $  0.2688 $ &  $ -0.0325 $ &  $  0.0031 $ &  $  0.0000 $ & $   0.003 $ \\
$uvw1 - J$ &  $(-2.84, 3.77)$ &  $ -0.0993 $ &  $  0.3580 $ &  $ -0.0656 $ &  $  0.0102 $ &  $ -0.0002 $ & $   0.003 $ \\
$u - J$ &  $(-2.37, 2.78)$ &  $  0.1786 $ &  $  0.3785 $ &  $ -0.1028 $ &  $  0.0327 $ &  $ -0.0051 $ & $   0.002 $ \\
$b - J$ &  $(-0.50, 1.53)$ &  $ -0.3026 $ &  $  1.8880 $ &  $ -1.8148 $ &  $  1.1562 $ &  $ -0.3011 $ & $   0.005 $ \\
$v - J$ &  $(-0.15, 0.68)$ &  $ -0.5162 $ &  $  6.0389 $ &  $ -15.2556 $ &  $ 22.7081 $ &  $ -13.3397 $ & $   0.007 $ \\
$g - H$ &  $(-0.25, 1.75)$ &  $ -0.6188 $ &  $  3.6820 $ &  $ -4.2535 $ &  $  2.7325 $ &  $ -0.6751 $ & $   0.018 $ \\
$r - H$ &  $(-0.04, 0.73)$ &  $ -1.4116 $ &  $ 11.7645 $ &  $ -28.5267 $ &  $ 36.5778 $ &  $ -17.9388 $ & $   0.015 $ \\
$i - H$ &  $( 0.26, 0.69)$ &  $ -13.5662 $ &  $ 77.7477 $ &  $ -162.4656 $ &  $ 149.4979 $ &  $ -47.3722 $ & $   0.025 $ \\
$uvw2 - H$ &  $(-3.04, 4.82)$ &  $ -0.1736 $ &  $  0.3471 $ &  $ -0.0499 $ &  $  0.0052 $ &  $  0.0000 $ & $   0.005 $ \\
$uvm2 - H$ &  $(-3.79, 5.19)$ &  $ -0.1436 $ &  $  0.2814 $ &  $ -0.0327 $ &  $  0.0030 $ &  $  0.0000 $ & $   0.003 $ \\
$uvw1 - H$ &  $(-2.78, 3.93)$ &  $ -0.0396 $ &  $  0.3791 $ &  $ -0.0665 $ &  $  0.0099 $ &  $ -0.0002 $ & $   0.003 $ \\
$u - H$ &  $(-2.31, 2.94)$ &  $  0.2430 $ &  $  0.4136 $ &  $ -0.1089 $ &  $  0.0327 $ &  $ -0.0047 $ & $   0.002 $ \\
$b - H$ &  $(-0.45, 1.69)$ &  $ -0.3893 $ &  $  2.1448 $ &  $ -1.8865 $ &  $  1.0618 $ &  $ -0.2433 $ & $   0.004 $ \\
$v - H$ &  $(-0.09, 0.83)$ &  $ -0.9573 $ &  $  7.5451 $ &  $ -15.4278 $ &  $ 17.5308 $ &  $ -7.8327 $ & $   0.006 $ \\
$g - K$ &  $(-0.15, 2.03)$ &  $ -0.9482 $ &  $  4.5328 $ &  $ -4.5543 $ &  $  2.2909 $ &  $ -0.4268 $ & $   0.025 $ \\
$r - K$ &  $( 0.07, 1.01)$ &  $ -2.7865 $ &  $ 17.7213 $ &  $ -35.5258 $ &  $ 34.5439 $ &  $ -12.5417 $ & $   0.016 $ \\
$i - K$ &  $( 0.36, 0.97)$ &  $ -26.5438 $ &  $ 142.2930 $ &  $ -289.7638 $ &  $ 269.8118 $ &  $ -94.6030 $ & $   0.039 $ \\
$uvw2 - K$ &  $(-2.94, 4.89)$ &  $ -0.1083 $ &  $  0.3564 $ &  $ -0.0515 $ &  $  0.0052 $ &  $  0.0000 $ & $   0.004 $ \\
$uvm2 - K$ &  $(-3.69, 5.25)$ &  $ -0.0715 $ &  $  0.2873 $ &  $ -0.0336 $ &  $  0.0030 $ &  $  0.0000 $ & $   0.003 $ \\
$uvw1 - K$ &  $(-2.68, 4.00)$ &  $  0.0220 $ &  $  0.3918 $ &  $ -0.0697 $ &  $  0.0100 $ &  $ -0.0002 $ & $   0.003 $ \\
$u - K$ &  $(-2.21, 3.01)$ &  $  0.2998 $ &  $  0.4342 $ &  $ -0.1201 $ &  $  0.0345 $ &  $ -0.0048 $ & $   0.002 $ \\
$b - K$ &  $(-0.34, 1.76)$ &  $ -0.5265 $ &  $  2.5676 $ &  $ -2.2418 $ &  $  1.1747 $ &  $ -0.2494 $ & $   0.004 $ \\
$v - K$ &  $( 0.01, 0.90)$ &  $ -1.8154 $ &  $ 11.4063 $ &  $ -21.7712 $ &  $ 21.5404 $ &  $ -8.3255 $ & $   0.005 $ \\
$g - r$ &  $(-0.21, 1.02)$ &  $ -0.3017 $ &  $  4.0452 $ &  $ -10.4765 $ &  $ 12.3446 $ &  $ -5.2003 $ & $   0.026 $ \\
$g - i$ &  $(-0.51, 1.07)$ &  $ -0.0271 $ &  $  1.2274 $ &  $ -2.7411 $ &  $  4.1534 $ &  $ -2.1262 $ & $   0.025 $ \\
$g - z$ &  $(-0.77, 1.29)$ &  $ -0.0218 $ &  $  0.8763 $ &  $ -1.1897 $ &  $  1.5281 $ &  $ -0.6293 $ & $   0.026 $ \\
$uvw2 - g$ &  $(-2.79, 3.61)$ &  $ -0.2858 $ &  $  0.2236 $ &  $ -0.0633 $ &  $  0.0066 $ &  $ -0.0007 $ & $   0.003 $ \\
$uvm2 - g$ &  $(-3.55, 3.99)$ &  $ -0.2716 $ &  $  0.1757 $ &  $ -0.0412 $ &  $  0.0032 $ &  $ -0.0002 $ & $   0.002 $ \\
$uvw1 - g$ &  $(-2.53, 2.73)$ &  $ -0.1961 $ &  $  0.2142 $ &  $ -0.0882 $ &  $  0.0121 $ &  $ -0.0022 $ & $   0.005 $ \\
$u - g$ &  $(-2.06, 1.74)$ &  $ -0.0612 $ &  $  0.0812 $ &  $ -0.1371 $ &  $  0.0543 $ &  $ -0.0165 $ & $   0.001 $ \\
$b - g$ &  $(-0.20, 0.49)$ &  $ -0.2215 $ &  $  2.6298 $ &  $ -14.1060 $ &  $ 31.4305 $ &  $ -27.5948 $ & $   0.007 $ \\
$g - v$ &  $(-0.16, 0.36)$ &  $ -0.3333 $ &  $  4.9729 $ &  $ -19.2272 $ &  $ 40.8964 $ &  $ -41.9869 $ & $   0.001 $ \\
$r - z$ &  $(-0.56, 0.27)$ &  $  0.3686 $ &  $  1.5409 $ &  $  0.8795 $ &  $ -2.6287 $ &  $ -26.5600 $ & $   0.023 $ \\
$uvw2 - r$ &  $(-3.01, 4.18)$ &  $ -0.2826 $ &  $  0.2836 $ &  $ -0.0538 $ &  $  0.0061 $ &  $ -0.0002 $ & $   0.001 $ \\
$uvm2 - r$ &  $(-3.76, 4.54)$ &  $ -0.2653 $ &  $  0.2284 $ &  $ -0.0351 $ &  $  0.0032 $ &  $ -0.0001 $ & $   0.001 $ \\
$uvw1 - r$ &  $(-2.75, 3.29)$ &  $ -0.1645 $ &  $  0.2965 $ &  $ -0.0725 $ &  $  0.0115 $ &  $ -0.0007 $ & $   0.001 $ \\
$u - r$ &  $(-2.28, 2.30)$ &  $  0.0658 $ &  $  0.2650 $ &  $ -0.1104 $ &  $  0.0401 $ &  $ -0.0081 $ & $   0.002 $ \\
$b - r$ &  $(-0.41, 1.05)$ &  $ -0.2432 $ &  $  1.8866 $ &  $ -3.1239 $ &  $  3.0317 $ &  $ -1.2002 $ & $   0.005 $ \\
$i - z$ &  $(-0.26, 0.23)$ &  $  0.3890 $ &  $  2.9310 $ &  $ -9.1123 $ &  $ 36.5702 $ &  $ -143.3480 $ & $   0.055 $ \\
$uvw2 - i$ &  $(-3.31, 4.13)$ &  $ -0.4509 $ &  $  0.2759 $ &  $ -0.0476 $ &  $  0.0058 $ &  $ -0.0000 $ & $   0.003 $ \\
$uvm2 - i$ &  $(-4.06, 4.50)$ &  $ -0.4456 $ &  $  0.2269 $ &  $ -0.0314 $ &  $  0.0033 $ &  $  0.0000 $ & $   0.002 $ \\
$uvw1 - i$ &  $(-3.05, 3.24)$ &  $ -0.3223 $ &  $  0.2867 $ &  $ -0.0609 $ &  $  0.0109 $ &  $ -0.0004 $ & $   0.002 $ \\
$u - i$ &  $(-2.58, 2.25)$ &  $ -0.0747 $ &  $  0.2652 $ &  $ -0.0786 $ &  $  0.0309 $ &  $ -0.0066 $ & $   0.002 $ \\
$b - i$ &  $(-0.71, 1.00)$ &  $ -0.1679 $ &  $  0.9603 $ &  $ -1.1771 $ &  $  1.3439 $ &  $ -0.6621 $ & $   0.006 $ \\
$v - i$ &  $(-0.36, 0.15)$ &  $  0.1819 $ &  $  1.4336 $ &  $ -0.0497 $ &  $ -14.7618 $ &  $ -147.1774 $ & $   0.016 $ \\
$uvw2 - z$ &  $(-3.57, 4.11)$ &  $ -0.5703 $ &  $  0.2814 $ &  $ -0.0423 $ &  $  0.0054 $ &  $ -0.0000 $ & $   0.004 $ \\
$uvm2 - z$ &  $(-4.32, 4.49)$ &  $ -0.5728 $ &  $  0.2350 $ &  $ -0.0283 $ &  $  0.0031 $ &  $  0.0000 $ & $   0.002 $ \\
$uvw1 - z$ &  $(-3.31, 3.23)$ &  $ -0.4292 $ &  $  0.2947 $ &  $ -0.0521 $ &  $  0.0098 $ &  $ -0.0003 $ & $   0.003 $ \\
$u - z$ &  $(-2.84, 2.23)$ &  $ -0.1557 $ &  $  0.2865 $ &  $ -0.0641 $ &  $  0.0231 $ &  $ -0.0054 $ & $   0.002 $ \\
$b - z$ &  $(-0.97, 0.98)$ &  $ -0.1868 $ &  $  0.7817 $ &  $ -0.5750 $ &  $  0.6121 $ &  $ -0.3492 $ & $   0.005 $ \\
$v - z$ &  $(-0.62, 0.13)$ &  $  0.1972 $ &  $  1.0516 $ &  $ -2.0903 $ &  $ -7.5558 $ &  $ -19.8028 $ & $   0.007 $ \\
$uvw2 - uvw1$ &  $(-0.26, 0.88)$ &  $  0.7871 $ &  $ -1.2202 $ &  $ -2.1603 $ &  $  0.8002 $ &  $ -0.5491 $ & $   0.003 $ \\
$uvw2 - u$ &  $(-0.73, 1.84)$ &  $  0.7359 $ &  $  0.1051 $ &  $ -0.3231 $ &  $  0.0273 $ &  $ -0.0114 $ & $   0.002 $ \\
$uvw2 - b$ &  $(-2.60, 3.11)$ &  $ -0.2695 $ &  $  0.1687 $ &  $ -0.0765 $ &  $  0.0063 $ &  $ -0.0014 $ & $   0.005 $ \\
$uvw2 - v$ &  $(-2.95, 3.98)$ &  $ -0.2753 $ &  $  0.2711 $ &  $ -0.0561 $ &  $  0.0060 $ &  $ -0.0004 $ & $   0.002 $ \\
$uvm2 - uvw1$ &  $(-1.01, 1.26)$ &  $  0.4121 $ &  $ -1.0084 $ &  $ -0.4250 $ &  $  0.0252 $ &  $ -0.0271 $ & $   0.002 $ \\
$uvm2 - u$ &  $(-1.48, 2.22)$ &  $  0.7378 $ &  $ -0.0634 $ &  $ -0.1501 $ &  $  0.0050 $ &  $ -0.0029 $ & $   0.002 $ \\
$uvm2 - b$ &  $(-3.35, 3.48)$ &  $ -0.2577 $ &  $  0.1272 $ &  $ -0.0492 $ &  $  0.0027 $ &  $ -0.0005 $ & $   0.003 $ \\
$uvm2 - v$ &  $(-3.70, 4.35)$ &  $ -0.2577 $ &  $  0.2172 $ &  $ -0.0368 $ &  $  0.0031 $ &  $ -0.0001 $ & $   0.002 $ \\
$uvw1 - u$ &  $(-0.47, 0.97)$ &  $  0.7393 $ &  $  0.1369 $ &  $ -0.8568 $ &  $  0.0766 $ &  $ -0.0716 $ & $   0.001 $ \\
$uvw1 - b$ &  $(-2.34, 2.23)$ &  $ -0.2082 $ &  $  0.1320 $ &  $ -0.1140 $ &  $  0.0093 $ &  $ -0.0048 $ & $   0.007 $ \\
$uvw1 - v$ &  $(-2.69, 3.10)$ &  $ -0.1640 $ &  $  0.2796 $ &  $ -0.0763 $ &  $  0.0111 $ &  $ -0.0012 $ & $   0.003 $ \\
$u - b$ &  $(-1.87, 1.25)$ &  $ -0.2020 $ &  $ -0.1606 $ &  $ -0.1979 $ &  $  0.0574 $ &  $ -0.0354 $ & $   0.001 $ \\
$u - v$ &  $(-2.22, 2.11)$ &  $  0.0455 $ &  $  0.2232 $ &  $ -0.1231 $ &  $  0.0413 $ &  $ -0.0098 $ & $   0.001 $ \\
$b - v$ &  $(-0.35, 0.85)$ &  $ -0.2540 $ &  $  2.0811 $ &  $ -4.1806 $ &  $  4.5357 $ &  $ -2.1469 $ & $   0.003 $ \\

